VisTabNet: Adapting Vision Transformers for Tabular Data

Although deep learning models have had great success in natural language processing and computer vision, we do not observe comparable improvements in the case of tabular data, which is still the most common data type used in biological, industrial and financial applications. In particular, it is challenging to transfer large-scale pre-trained models to downstream tasks defined on small tabular datasets. To address this, we propose VisTabNet -- a cross-modal transfer learning method, which allows for adapting Vision Transformer (ViT) with pre-trained weights to process tabular data. By projecting tabular inputs to patch embeddings acceptable by ViT, we can directly apply a pre-trained Transformer Encoder to tabular inputs. This approach eliminates the conceptual cost of designing a suitable architecture for processing tabular data, while reducing the computational cost of training the model from scratch. Experimental results on multiple small tabular datasets (less than 1k samples) demonstrate VisTabNet's superiority, outperforming both traditional ensemble methods and recent deep learning models. The proposed method goes beyond conventional transfer learning practice and shows that pre-trained image models can be transferred to solve tabular problems, extending the boundaries of transfer learning. We share our example implementation as a GitHub repository available at https://github.com/wwydmanski/VisTabNet.

==> old/TODO.tex <==
do Ulviego: większe zbiory:
-https://www.openml.org/d/44130
-https://www.openml.org/d/44122
-https://www.openml.org/d/44162
-https://www.openml.org/d/44158
-https://www.openml.org/d/44156


marek: wszystkie eksperymenty robimy na datasetach:
-Cylinder Bands
-Credit approval
-dermatology
-libras 
-zoo
-Volkert (były w pracy z hypertab)
-Nomao (były w pracy z hypertab)

Zadania:
(ulvi) 1. puścić na większych zbiorach
(ulvi) 2. więcej zbiorów w tabelce 3 gdzie jest finetuning3
(ulvi) 3. wykres jak zmienia się acc wraz z biegiem finetuningu
(witek) 4. Inne architektury (ok 5 zbiorów)
-ResNet z obrazków
-BERT *
-fully-connected pretrenowany na MNIST albo CIFAR *
-fully-connected _niepretrenowany_
-ViT niepretrenowany na niczym (tylko zainicjalizowany losowo) *
4.1 
 - dodać info o architekturze pretrenowanego transformera
 - dodać ranking do tab 5. *
(witek) 5 Ablacja c.d
-czy więcej warstw w adapterze warto dawac *
-Focal loss vs. cross entropy *
-czy więcej warstw dla heada klasyfikacyjnego *
6 (witek) Zmienić setting few-shot na jakieś dane tabelaryczne *
 - porównanie: pozostałe metody z tabelki 2 *

-------------------------------------

(ulvi implementuje, witek review kodu) rzutowanie w różne warstwy enkodera - obecnie rzutujemy na pierwszą ale nic nie stoi na przeszkodzie żeby rzutować na 0, 2, 4, 6 itd. Podobnie można wychodzić wcześniej niż z ostatniej warstyw enkodera (head klasyfikacyjny przykładamy do wartstwy n, n-2, n-4, n-6, itd. Zrobimy wykres accuracy, gdzie na osi x będzie nr warstwy do której rzutujemy (albo z której wychodzimy). Bierzemy takie same 5 zbiorów jak poprzednio.


---------------

<-typowe podejście do trasfer learnngu - pretrening i finetuning
<-my startujemy od bazowego modelu


--- Ulvi
1)
- Wyraźnie określic, dlaczego adaptacja ViT do danych tabelarycznych jest istotna, poza wspomnieniem ich sukcesu w innych dziedzinach. Podkreślic moze konkretne wyzwania związane z danymi tabelarycznymi i jak VisTabNet je rozwiązuje.
2)
- Moze wiecej skoncentrowac się szczególnie na tym, dlaczego wcześniejsze próby z transformatorami w danych tabelarycznych nie przyniosły oczekiwanych rezultatów i jak VisTabNet pokonuje te problemy.
3)
- Podac więcej szczegółów technicznych i uzasadnienia dla architektury VisTabNet. Moze dodac nowy obraz
- Rozwińac uzasadnienie stosowania Focal Loss, augmentacji danych przez dodanie szumu oraz zróżnicowanych współczynników uczenia. Dodac / wymislic więcej matematycznych wzorów moze wzbogacic ta ciesc 
4)
- Summary in dataset: Mamy 16 zbiorów danych binarnych oraz 7 wieloklasowych. Możemy zmniejszyć tę liczbę do 7 vs 7, albo zwiększyć do 16 vs 16, aby pokazać uniwersalność - zbalansowanosc podejścia w klasyfikacji.
- 542-546 napewno to robimy?
- Mozemy sprobowac uwzglednic badania ablacyjne, aby pokazać wkład każdego komponentu (np. warstwy adaptacyjnej, Focal Loss) w ogólną wydajność.
- Mozemy sprawdzic wrażliwość na hiperparametry: Przeanalizowac, jak wrażliwy jest VisTabNet na zmiany hiperparametrów i podac rekomendacje dotyczące optymalnych ustawień.
- Wydaje mi się, że w liniach 571 - 577 jest błąd, ponieważ Node nie jest drugim najlepszym głębokim modelem. Drugim najlepszym jest FT. Node jest na 5 miejscu. Linie 668 - 669 też mówią trochę inne rzeczy - mogą być nieczytelne.

-- Witek
- (przemyśleć) Zmienić setting few-shot na jakieś dane tabelaryczne
- Dodać szczegóły treningu NN w głównym papierze
- 
